Projecting Non-Fungible Token (NFT) Collections: A Contextual Generative Approach

Non-fungible tokens (NFTs) are digital assets stored on a blockchain representing real-world objects such as art or collectibles. An NFT collection comprises numerous tokens; each token can be transacted multiple times. It is a multibillion-dollar market where the number of collections has more than doubled in 2022. In this paper, we want to obtain a generative model that, given the early transactions history (first quarter Q1) of a newly minted collection, generates subsequent transactions (quarters Q2, Q3, Q4), where the generative model is trained using the transaction history of a few mature collections. The goal is to use the generated transactions to project the potential market value of this newly minted collection over the next few quarters. A technical challenge exists in that different collections have diverse characteristics, and the generative model should generate based on the appropriate "contexts" of the collection. Our method takes a two-step approach. First, it employs unsupervised learning on the early transactions to extract characteristics (which we call contexts) of NFT collections. Next, it generates future transactions of each token based on these contexts and the early transactions, projecting the target collection's potential market value. Comprehensive experiments demonstrate our contextual generative approach's NFT projection capabilities.

==> input/old/tab-baseline.tex <==
% =========================================
\begin{table}[!htbp]
\centering
\caption{LSTM prediction.}
\resizebox{0.99\linewidth}{!}{%
    \begin{tabular}{|c|c|ccc|c|}
    \hline
    \multirow{2}{*}{\textbf{NFT Collection}} & \multirow{2}{*}{\textbf{Tier (actual)}} &\multicolumn{3}{c|}{\textbf{Quarter}} & \multirow{2}{*}{\textbf{Tier (predict)}} \\ %\cline{3-7}
    & & \textbf{\nth{2}} & \textbf{\nth{3}} & \textbf{\nth{4}} & \multicolumn{1}{c|}{}
     \\ \hline 
    
    % & &\multicolumn{5}{c}{Actual} \\ \cline{2-7}
    \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}\textit{Collection}  \\ \end{tabular}}
        % \rule{0pt}{3ex}   &$A$  &&&\multicolumn{1}{l|}{} &2   \\ 
        % \rule{0pt}{3ex}   &$B$  &&&\multicolumn{1}{l|}{} &4  \\
        \rule{0pt}{3ex}   &$1$  & & &       &3   \\ \hline 
    \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}\textit{NEKO}  \\ \end{tabular}}
        % \rule{0pt}{3ex}   &$A$ &&&\multicolumn{1}{l|}{} &5  \\
        % \rule{0pt}{3ex}   &$B$ &&&\multicolumn{1}{l|}{} &1 \\
        \rule{0pt}{3ex}   &$4$ & & &        &5  \\ \hline
    \end{tabular}
}
% \linebreak
\label{tab:baselineperf}
\end{table} 


==> input/old/tab-replicate.tex <==
% =========================================
\begin{table}[!htbp]
\centering
\caption{table}{Generating observed networks.}
\resizebox{0.99\linewidth}{!}{%
    \begin{tabular}{c|c|ccccc}
    % \hline
    \textbf{NFT Collection} & \textbf{Quarter} & \textbf{Stat1} & \textbf{Stat2} & \textbf{Stat3} & \textbf{Stat4} & \textbf{Stat5} \\ \hline 
    
    % & &\multicolumn{5}{c}{Actual} \\ \cline{2-7}
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textit{BAYC}  \end{tabular}}
        \rule{0pt}{3ex}   &$\nth{2}$  &&&&& \\ 
        \rule{0pt}{3ex}   &$\nth{3}$  &&&&& \\
        \rule{0pt}{3ex}   &$\nth{4}$  &&&&& \\ \hline 
    
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textit{Hashmasks}  \end{tabular}}
        \rule{0pt}{3ex}   &$\nth{2}$ &&&&& \\
        \rule{0pt}{3ex}   &$\nth{3}$ &&&&& \\ %\\
        \rule{0pt}{3ex}   &$\nth{4}$ &&&&& \\ \hline
        
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textit{Chubbies}  \end{tabular}}
        \rule{0pt}{3ex}   &$\nth{2}$  &&&&&  \\
        \rule{0pt}{3ex}   &$\nth{3}$  &&&&& \\ 
        \rule{0pt}{3ex}   &$\nth{4}$  &&&&& \\ \hline
    
    \end{tabular}
}
% \linebreak
\label{tab:replicate}
% \end{figure} 
\end{table} 

==> input/tab-perf.tex <==
% =========================================
\begin{table*}[!htbp]
\centering
\caption{Performance measures (regression statistics and market metrics) of the transaction series generated by our contextual generative models, ContextPred and NFTContextPred, and the baseline single collection models. Values that reflect the best performance are in bold. Our contextual approach mostly achieves the highest regression statistics and closely matches the actual market metrics compared to the baseline models.}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{c|c|cccccccc|c}
    % \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{NFT Collection} \end{tabular}}
    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Model} \end{tabular}}
    & \multicolumn{4}{c}{\textbf{Regression Stats}} & \multicolumn{4}{c}{\textbf{Market Cap}} & \textbf{Tier} \\
    & &\textbf{MAE} & \textbf{MSE} & \textbf{RMSE} & $\mathbf{R^2}$ & $\mathbf{Q_1}$ & $\mathbf{Q_2}$ & $\mathbf{Q_3}$ & $\mathbf{Q_4}$ & \\ \hline 

    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\textit{Chubbies}} \end{tabular}} 
        \rule{0pt}{3ex}   &Actual  &--&--&--&-- &3,132.28 &3,049.97 &2,967.42 &2,917.50 &2   \\ \cline{2-11}
        \rule{0pt}{3ex}   &$\mathcal{M}_{1}$   &46.80 &7,105.05 &84.29 &-5,132.98 &0.00 &22.96 &119.81 &579.10 &1   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{2}$   &0.41   &0.80 &0.89 &0.36 &0.00 &0.26  &0.29   &0.31 &\underline{2}   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{3}$   &0.26 &0.62  &0.79 &0.51 &0.00 &0.18  &0.27   &0.33 &3   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{4}$   &0.33 &1.07  &1.03 &0.14 &0.00 &0.87  &0.86   &0.86 &3   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{5}$   &0.35 &1.09  &1.05 &0.11 &0.00 &0.95  &0.95   &0.95 &3   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{\bf{X}}$  &0.35 &0.57  &0.76 &0.55 &0.00 &0.99  &0.99   &0.99 &3   \\
        \rule{0pt}{3ex}   &\emph{ContextPred} &0.32 &0.69  &0.83 &0.45 &0.00 &0.27  &0.25   &0.23 &\underline{2}   \\ %\cline{3-11}
        \rule{0pt}{3ex}   &\emph{NFT ContextPred}  &\bf{0.18} &\bf{0.23}  &\bf{0.48} &\bf{0.83} &0.00 &\bf{0.07}  &\bf{0.07}   &\bf{0.05} &\underline{2}   \\ \hline 
        
    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\textit{CryptoTrunks}}  \end{tabular}} 
        \rule{0pt}{3ex}   &Actual  &--&--&--&-- &1,250.64 &1,381.67 &1,383.83 &1,381.40 &3   \\ \cline{2-11}
        \rule{0pt}{3ex}   &$\mathcal{M}_{1}$   &46.29   &6,914.36 &83.15 &-11,045.39 &0.00 &30.18 &152.28 &726.26 &1   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{2}$   &0.38   &0.45 &0.67 &0.28 &0.00 &0.65  &0.64   &0.63 &2   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{3}$   &0.27 &\bf{0.34}  &\bf{0.58} &\bf{0.44} &0.00 &0.13  &0.17   &0.20 &\underline{3}   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{4}$   &0.26 &0.53  &0.73 &0.13 &0.00 &0.82  &0.82   &0.82 &\underline{3}   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{5}$   &0.27 &0.55  &0.74 &0.10 &0.00 &0.94  &0.94   &0.94 &\underline{3}   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{\bf{X}}$  &0.32 &0.52  &0.72 &0.16 &0.00 &1.18  &1.18   &1.17 &\underline{3}   \\
        \rule{0pt}{3ex}   &\emph{ContextPred}  &0.31 &0.43  &0.65 &0.31 &0.00 &\bf{0.04}  &\bf{0.04}   &\bf{0.03} &\underline{3}   \\ %\cline{3-11}
        \rule{0pt}{3ex}   &\emph{NFT CondPred}  &\bf{0.22} &0.35  &0.59 &\bf{0.44} &0.00 &0.13  &0.13   &0.14 &\underline{3}   \\ \hline
        
    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\textit{VeeFriends}}  \end{tabular}} 
        \rule{0pt}{3ex}   &Actual  &--&--&--&-- &22,287.76 &32,894.39 &37,948.39 &43,902.90 &1   \\ \cline{2-11}
        \rule{0pt}{3ex}   &$\mathcal{M}_{1}$   &53.78   &9,944.38   &99.72   &-190.46 &0.00 &3.31  &16.12  &61.27 &\underline{1}   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{2}$   &2.37   &49.04 &7.00 &-0.21 &0.00 &0.78  &0.84   &0.86 &2   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{3}$   &2.28 &34.26 &5.85 &0.12 &0.00 &0.72  &0.83   &0.91 &2   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{4}$   &2.88 &39.74 &6.30 &-0.05 &0.00 &0.98  &0.98   &0.99 &3   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{5}$   &2.91 &39.99 &6.32 &-0.06 &0.00 &0.99  &0.99   &1.00 &3   \\
        \rule{0pt}{3ex}   &$\mathcal{M}_{\bf{X}}$  &2.62 &33.72 &5.81 &0.16 &0.00 &0.92  &0.93   &0.94 &2   \\
        \rule{0pt}{3ex}   &\emph{ContextPred}  &2.24 &30.33 &5.51 &0.25 &0.00 &0.74  &0.77   &0.80 &\underline{1}   \\ %\cline{3-11}
        \rule{0pt}{3ex}   &\emph{NFT ContextPred}  &\bf{1.56} &\bf{24.45} &\bf{4.94} &\bf{0.40} &0.00 &\bf{0.49}  &\bf{0.57}   &\bf{0.62} &\underline{1}   \\ \hline         
        
        
\end{tabular}
}
% \linebreak
\label{tab:predictperf}
\end{table*} 
